Active spin lattice hyperpolarization: Application to hexagonal boron nitride color centers

The active driving of the electron spin of a color center is known as a method for the hyperpolarization of the surrounding nuclear spin bath and to initialize a system with large number of spins. Here, we investigate the efficiency of this approach for various spin coupling schemes in a one-dimensional Heisenberg chain coupled to a central spin. To extend our study to the realistic systems with a large number of interacting spins, we employ an approximate method based on Holstein-Primakoff transformation. The validity of the method for describing spin polarization dynamics is benchmarked by the exact numerics for a small lattice, where the accuracy of the bosonic Holstein-Primakoff approximation approach is confirmed. We, thus, extend our analysis to larger spin systems where the exact numerics are out of reach. The results prove the efficiency of the active driving method when the central spin interaction with the spin bath is long range and the inter-spin interactions in the bath spins is large enough. The method is then applied to the realistic case of optically active negatively charged boron vacancy centers ($V_B$) in hexagonal boron nitride. Our results suggest that a high degree of hyperpolarization in the boron and nitrogen nuclear spin lattices is achievable even starting from a fully thermal bath. As an initialization, our work provides the first step toward the realization of a two-dimensional quantum simulator based on natural nuclear spins and it can prove useful for extending the coherence time of the $V_B$ centers.

==> qip2d.tex <==
% Encoding: ISO-8859-1

@book{stoneham2001theory,
  title={Theory of defects in solids: electronic structure of defects in insulators
    and semiconductors},
  author={Stoneham, Arthur Marshall},
  year={2001},
  publisher={Oxford University Press}
}

@Article{Doherty2013,
  author={Marcus W. Doherty and Neil B. Manson and Paul Delaney and Fedor Jelezko
    and J{\~A}¶rg Wrachtrup and Lloyd C.L. Hollenberg},
  journal={Phys. Rep.},
  title={The nitrogen-vacancy colour centre in diamond},
  year={2013},
  month={jul},
  number={1},
  pages={1--45},
  volume={528},
  doi={10.1016/j.physrep.2013.02.001},
  owner={Mehdi Abdi},
  publisher={Elsevier {BV}}
}

@Article{dolde2014high,
  author    = {Dolde, Florian and Bergholm, Ville and Wang, Ya and Jakobi, Ingmar and Naydenov, Boris and Pezzagna, S{\'e}bastien and Meijer, Jan and Jelezko, Fedor and Neumann, Philipp and Schulte-Herbr{\"u}ggen, Thomas and others},
  journal   = {Nat. Commun.},
  title     = {High-fidelity spin entanglement using optimal control},
  year      = {2014},
  number    = {1},
  pages     = {3371},
  volume    = {5},
  doi       = {https://doi.org/10.1038/ncomms4371},
  publisher = {Nature Publishing Group},
}

@article{pla2013high,
  title={High-fidelity readout and control of a nuclear spin qubit in silicon},
  author={Pla, Jarryd J and Tan, Kuan Y and Dehollain, Juan P and Lim, Wee H and
    Morton, John JL and Zwanenburg, Floris A and Jamieson, David N and Dzurak,
    Andrew S and Morello, Andrea},
  journal={Nature},
  volume={496},
  number={7445},
  pages={334--338},
  year={2013},
  publisher={Nature Publishing Group},
  doi={https://doi.org/10.1038/nature12011}
}

@article{jelezko2004observation,
  title={Observation of coherent oscillation of a single nuclear spin and realization
    of a two-qubit conditional quantum gate},
  author={Jelezko, Fedor and Gaebel, T and Popa, I and Domhan, M and Gruber, A
    and Wrachtrup, Jorg},
  journal={Phys. Rev. Lett.},
  volume={93},
  number={13},
  pages={130501},
  year={2004},
  publisher={APS},
  doi={https://doi.org/10.1103/PhysRevLett.93.130501}
}

@article{Cai2013,
  author={Jianming Cai and Alex Retzker and Fedor Jelezko and Martin B. Plenio},
  doi={10.1038/nphys2519},
  journal={Nat. Phys.},
  month={jan},
  number={3},
  owner={Mehdi Abdi},
  pages={168--173},
  publisher={Springer Science and Business Media {LLC}},
  title={A large-scale quantum simulator on a diamond surface at room temperature},
  volume={9},
  year={2013},
  bdsk-url-1={https://doi.org/10.1038/nphys2519}
}

@Article{unden2018coherent,
  author    = {Unden, Thomas and Tomek, Nikolas and Weggler, Timo and Frank, Florian and London, Paz and Zopes, Jonathan and Degen, Christian and Raatz, Nicole and Meijer, Jan and Watanabe, Hideyuki and others},
  journal   = {npj Quantum Inf.},
  title     = {Coherent control of solid state nuclear spin nano-ensembles},
  year      = {2018},
  number    = {1},
  pages     = {39},
  volume    = {4},
  doi       = {https://doi.org/10.1038/s41534-018-0089-8},
  publisher = {Nature Publishing Group},
}

@article{London2013,
  author={London, P. and Scheuer, J. and Cai, J.-M. and Schwarz, I. and Retzker,
    A. and Plenio, M. B. and Katagiri, M. and Teraji, T. and Koizumi, S. and Isoya,
    J. and Fischer, R. and McGuinness, L. P. and Naydenov, B. and Jelezko, F.},
  doi={10.1103/PhysRevLett.111.067601},
  issue={6},
  journal={Phys. Rev. Lett.},
  month={Aug},
  numpages={5},
  pages={067601},
  publisher={American Physical Society},
  title={Detecting and Polarizing Nuclear Spins with Double Resonance on a Single
    Electron Spin},
  url={https://link.aps.org/doi/10.1103/PhysRevLett.111.067601},
  volume={111},
  year={2013},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevLett.111.067601},
  bdsk-url-2={https://doi.org/10.1103/PhysRevLett.111.067601}
}

@Article{Rej2015,
  author={Rej, Ewa and Gaebel, Torsten and Boele, Thomas and Waddington, David
    EJ and Reilly, David J},
  journal={Nat. Commun.},
  title={Hyperpolarized nanodiamond with long spin-relaxation times},
  year={2015},
  pages={8459},
  volume={6},
  bdsk-url-1={https://doi.org/10.1038/ncomms9459},
  doi={https://doi.org/10.1038/ncomms9459},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/ncomms9459}
}

@Article{Healey2021,
  author     = {Healey, A.J. and Hall, L.T. and White, G.A.L. and Teraji, T. and Sani, M.-A. and Separovic, F. and Tetienne, J.-P. and Hollenberg, L.C.L.},
  journal    = {Phys. Rev. Appl.},
  title      = {Polarization Transfer to External Nuclear Spins Using Ensembles of Nitrogen-Vacancy Centers},
  year       = {2021},
  month      = {May},
  pages      = {054052},
  volume     = {15},
  bdsk-url-1 = {https://link.aps.org/doi/10.1103/PhysRevApplied.15.054052},
  bdsk-url-2 = {https://doi.org/10.1103/PhysRevApplied.15.054052},
  doi        = {10.1103/PhysRevApplied.15.054052},
  issue      = {5},
  numpages   = {16},
  publisher  = {American Physical Society},
  url        = {https://link.aps.org/doi/10.1103/PhysRevApplied.15.054052},
}

@Article{Fernandez2018a,
  author={Fern{\'a}ndez-Acebal, P. and Rosolio, O. and Scheuer, J. and M{\"u}ller,
    C. and M{\"u}ller, S. and Schmitt, S. and McGuinness, L.P. and Schwarz, I.
    and Chen, Q. and Retzker, A. and Naydenov, B. and Jelezko, F. and Plenio, M.B.},
  journal={Nano Lett.},
  title={Toward Hyperpolarization of Oil Molecules via Single Nitrogen Vacancy
    Centers in Diamond},
  year={2018},
  number={3},
  pages={1882-1887},
  volume={18},
  bdsk-url-1={https://doi.org/10.1021/acs.nanolett.7b05175},
  date-modified={2022-05-15 08:40:28 +0430},
  doi={10.1021/acs.nanolett.7b05175},
  url={https://doi.org/10.1021/acs.nanolett.7b05175}
}

@Article{alvarez2015local,
  author    = {{\'A}lvarez, Gonzalo A and Bretschneider, Christian O and Fischer, Ran and London, Paz and Kanda, Hisao and Onoda, Shinobu and Isoya, Junichi and Gershoni, David and Frydman, Lucio},
  journal   = {Nat. Commun.},
  title     = {Local and bulk 13C hyperpolarization in nitrogen-vacancy-centred diamonds at variable fields and orientations},
  year      = {2015},
  number    = {1},
  pages     = {8456},
  volume    = {6},
  doi       = {https://doi.org/10.1038/ncomms9456},
  publisher = {Nature Publishing Group},
}

@Article{king2015room,
  author    = {King, Jonathan P and Jeong, Keunhong and Vassiliou, Christophoros C and Shin, Chang S and Page, Ralph H and Avalos, Claudia E and Wang, Hai-Jing and Pines, Alexander},
  journal   = {Nat. Commun.},
  title     = {Room-temperature in situ nuclear spin hyperpolarization from optically pumped nitrogen vacancy centres in diamond},
  year      = {2015},
  number    = {1},
  pages     = {8965},
  volume    = {6},
  doi       = {https://doi.org/10.1038/ncomms9965},
  publisher = {Nature Publishing Group},
}

@Article{Scheuer2016,
  author={Jochen Scheuer and Ilai Schwartz and Qiong Chen and David Schulze-Sunninghausen
    and Patrick Carl and Peter Hofer and Alexander Retzker and Hitoshi Sumiya and
    Junichi Isoya and Burkhard Luy and Martin B Plenio and Boris Naydenov and Fedor
    Jelezko},
  journal={New J. Phys.},
  title={Optically induced dynamic nuclear spin polarisation in diamond},
  year={2016},
  month={jan},
  number={1},
  pages={013040},
  volume={18},
  bdsk-url-1={https://doi.org/10.1088/1367-2630/18/1/013040},
  date-modified={2022-05-15 08:42:27 +0430},
  doi={10.1088/1367-2630/18/1/013040},
  publisher={{IOP} Publishing},
  url={https://doi.org/10.1088/1367-2630/18/1/013040}
}

@Article{Ivady2020,
  author={Iv{\'a}dy, Viktor and Barcza, Gergely and Thiering, Gerg{\H{o}} and Li,
    Song and Hamdi, Hanen and Chou, Jyh-Pin and Legeza, {\"O}rs and Gali, Adam},
  journal={npj Comput. Mater.},
  title={Ab initio theory of the negatively charged boron vacancy qubit in hexagonal
    boron nitride},
  year={2020},
  pages={41},
  volume={6},
  bdsk-url-1={https://doi.org/10.1038/s41524-020-0305-x},
  doi={https://doi.org/10.1038/s41524-020-0305-x},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/s41524-020-0305-x}
}

@Article{Gottscholl2020,
  author={Gottscholl, Andreas and Kianinia, Mehran and Soltamov, Victor and Orlinskii,
    Sergei and Mamin, Georgy and Bradac, Carlo and Kasper, Christian and Krambrock,
    Klaus and Sperlich, Andreas and Toth, Milos and others},
  journal={Nat. Mater.},
  title={Initialization and read-out of intrinsic spin defects in a van der Waals
    crystal at room temperature},
  year={2020},
  number={5},
  pages={540--545},
  volume={19},
  bdsk-url-1={https://doi.org/10.1038/s41563-020-0619-6},
  doi={https://doi.org/10.1038/s41563-020-0619-6},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/s41563-020-0619-6}
}

@article{Kianinia2020,
  author={Kianinia, Mehran and White, Simon and Fr{\"o}ch, Johannes E and Bradac,
    Carlo and Aharonovich, Igor},
  journal={arXiv preprint arXiv:2004.07968},
  title={Engineering spin defects in hexagonal boron nitride},
  url={https://arxiv.org/abs/2004.07968},
  year={2020},
  bdsk-url-1={https://arxiv.org/abs/2004.07968}
}

@Article{gao2022nuclear,
  author    = {Xingyu Gao and Sumukh Vaidya and Kejun Li and Peng Ju and Boyang Jiang and Zhujing Xu and Andres E. Llacsahuanga Allcca and Kunhong Shen and Takashi Taniguchi and Kenji Watanabe and Sunil A. Bhave and Yong P. Chen and Yuan Ping and Tongcang Li},
  journal   = {Nat. Mater.},
  title     = {Nuclear spin polarization and control in a van der Waals material},
  year      = {2022},
  pages     = {1024-1028},
  volume    = {21},
  doi       = {https://doi.org/10.1038/s41563-022-01329-8},
  publisher = {Nature Publishing Group},
  url       = {https://doi.org/10.1038/s41563-022-01329-8},
}

@Article{Gottscholl2021,
  author={Andreas Gottscholl and Matthias Diez and Victor Soltamov and Christian
    Kasper and Andreas Sperlich and Mehran Kianinia and Carlo Bradac and Igor Aharonovich
    and Vladimir Dyakonov},
  journal={Sci. Adv.},
  title={Room temperature coherent control of spin defects in hexagonal boron nitride},
  year={2021},
  number={14},
  pages={3630},
  volume={7},
  abstract={Atomic defects in 2D materials show excellent spin coherence time and
    become promising contenders for quantum applications. Optically active spin
    defects are promising candidates for solid-state quantum information and sensing
    applications. To use these defects in quantum applications coherent manipulation
    of their spin state is required. Here, we realize coherent control of ensembles
    of boron vacancy centers in hexagonal boron nitride (hBN). Specifically, by
    applying pulsed spin resonance protocols, we measure a spin-lattice relaxation
    time of 18 microseconds and a spin coherence time of 2 microseconds at room
    temperature. The spin-lattice relaxation time increases by three orders of
    magnitude at cryogenic temperature. By applying a method to decouple the spin
    state from its inhomogeneous nuclear environment the optically detected magnetic
    resonance linewidth is substantially reduced to several tens of kilohertz.
    Our results are important for the employment of van der Waals materials for
    quantum technologies, specifically in the context of high resolution quantum
    sensing of two-dimensional heterostructures, nanoscale devices, and emerging
    atomically thin magnets.},
  bdsk-url-1={https://www.science.org/doi/abs/10.1126/sciadv.abf3630},
  bdsk-url-2={https://doi.org/10.1126/sciadv.abf3630},
  doi={10.1126/sciadv.abf3630},
  url={https://www.science.org/doi/abs/10.1126/sciadv.abf3630}
}

@Article{Tabesh2021,
  author        = {F T Tabesh and Q Hassanzada and M Hadian and A Hashemi and I Abdolhosseini Sarsari and M Abdi},
  journal       = {Quantum Sci. Technol.},
  title         = {Strain induced coupling and quantum information processing with hexagonal boron nitride quantum emitters},
  year          = {2021},
  month         = {oct},
  number        = {1},
  pages         = {015002},
  volume        = {7},
  bdsk-url-1    = {https://doi.org/10.1088/2058-9565/ac2f4d},
  date-modified = {2022-05-15 08:42:33 +0430},
  doi           = {10.1088/2058-9565/ac2f4d},
  publisher     = {{IOP} Publishing},
  url           = {https://doi.org/10.1088/2058-9565/ac2f4d},
}

@Article{Johansson2012,
  author={J.R. Johansson and P.D. Nation and Franco Nori},
  journal={Comput. Phys. Commun.},
  title={QuTiP: An open-source Python framework for the dynamics of open quantum
    systems},
  year={2012},
  issn={0010-4655},
  number={8},
  pages={1760-1772},
  volume={183},
  bdsk-url-1={https://www.sciencedirect.com/science/article/pii/S0010465512000835},
  bdsk-url-2={https://doi.org/10.1016/j.cpc.2012.02.021},
  date-modified={2022-05-15 08:41:11 +0430},
  doi={https://doi.org/10.1016/j.cpc.2012.02.021},
  keywords={Open quantum systems, Lindblad master equation, Quantum Monte Carlo,
    Python},
  url={https://www.sciencedirect.com/science/article/pii/S0010465512000835}
}

@article{Chen2015,
  author={Chen, Q. and Schwarz, I. and Jelezko, F. and Retzker, A. and Plenio,
    M. B.},
  doi={10.1103/PhysRevB.92.184420},
  issue={18},
  journal={Phys. Rev. B},
  month={Nov},
  numpages={18},
  pages={184420},
  publisher={American Physical Society},
  title={Optical hyperpolarization of $^{13}\mathrm{C}$ nuclear spins in nanodiamond
    ensembles},
  url={https://link.aps.org/doi/10.1103/PhysRevB.92.184420},
  volume={92},
  year={2015},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevB.92.184420},
  bdsk-url-2={https://doi.org/10.1103/PhysRevB.92.184420}
}

@article{Hartmann,
  author={Hartmann, S. R. and Hahn, E. L.},
  doi={10.1103/PhysRev.128.2042},
  issue={5},
  journal={Phys. Rev.},
  month={Dec},
  numpages={0},
  pages={2042--2053},
  publisher={American Physical Society},
  title={Nuclear Double Resonance in the Rotating Frame},
  url={https://link.aps.org/doi/10.1103/PhysRev.128.2042},
  volume={128},
  year={1962},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRev.128.2042},
  bdsk-url-2={https://doi.org/10.1103/PhysRev.128.2042}
}

@Book{Langhoff2012,
  editor={S. Langhoff},
  publisher={Springer Netherlands},
  title={Quantum Mechanical Electronic Structure Calculations with Chemical Accuracy},
  year={2012},
  isbn={9789401101936},
  date={2012-12-06},
  ean={9789401101936},
  owner={Mehdi Abdi},
  pagetotal={449}
}

@Article{Song2010,
  author={Li Song and Lijie Ci and Hao Lu and Pavel B. Sorokin and Chuanhong Jin
    and Jie Ni and Alexander G. Kvashnin and Dmitry G. Kvashnin and Jun Lou and
    Boris I. Yakobson and Pulickel M. Ajayan},
  journal={Nano Lett.},
  title={Large Scale Growth and Characterization of Atomic Hexagonal Boron Nitride
    Layers},
  year={2010},
  pages={3209--3215},
  volume={10},
  date-added={2022-05-15 08:36:32 +0430},
  date-modified={2022-05-15 08:38:59 +0430},
  doi={10.1021/nl1022139}
}

@article{Uhlenbeck1930,
  author={G. E. Uhlenbeck and L. S. Ornstein},
  date-added={2017-08-25 13:48:52 +0000},
  date-modified={2017-08-25 13:49:40 +0000},
  doi={10.1103/PhysRev.36.823},
  journal={Phys. Rev.},
  pages={823},
  title={On the Theory of the Brownian Motion},
  volume={36},
  year={1930},
  bdsk-url-1={https://doi.org/10.1103/PhysRev.36.823}
}

@article{Weissman1988,
  author={M. B. Weissman},
  date-added={2017-08-22 14:08:08 +0000},
  date-modified={2017-08-22 14:09:43 +0000},
  doi={10.1103/RevModPhys.60.537},
  journal={Rev. Mod. Phys.},
  pages={537--571},
  title={1/f noise and other slow, nonexponential kinetics in condensed matter},
  volume={60},
  year={1988},
  bdsk-url-1={https://doi.org/10.1103/RevModPhys.60.537}
}

@article{Bloch1957,
  author={F. Bloch},
  date-added={2017-08-22 13:47:45 +0000},
  date-modified={2017-08-22 13:48:30 +0000},
  doi={10.1103/PhysRev.105.1206},
  journal={Phys. Rev.},
  pages={1206},
  title={Generalized Theory of Relaxation},
  volume={105},
  year={1957},
  bdsk-url-1={https://doi.org/10.1103/PhysRev.105.1206}
}

@article{Paladino2014,
  author={E. Paladino and Y. M. Galperin and G. Falci and B. L. Altshuler},
  date-added={2017-08-22 09:15:04 +0000},
  date-modified={2017-08-22 09:16:42 +0000},
  doi={10.1103/RevModPhys.86.361},
  journal={Rev. Mod. Phys.},
  pages={361--418},
  title={1/f noise: Implications for solid-state quantum information},
  volume={86},
  year={2014},
  bdsk-url-1={https://doi.org/10.1103/RevModPhys.86.361}
}

@article{Yang2017,
  abstract={Decoherence of electron spins in nanoscale systems is important to
    quantum technologies such as quantum information processing and magnetometry.
    It is also an ideal model problem for studying the crossover between quantum
    and classical phenomena. At low temperatures or in light-element materials
    where the spin-orbit coupling is weak, the phonon scattering in nanostructures
    is less important and the fluctuations of nuclear spins become the dominant
    decoherence mechanism for electron spins. Since the 1950s, semi-classical noise
    theories have been developed for understanding electron spin decoherence. In
    spin-based solid-state quantum technologies, the relevant systems are in the
    nanometer scale and nuclear spin baths are quantum objects which require a
    quantum description. Recently, quantum pictures have been established to understand
    the decoherence and quantum many-body theories have been developed to quantitatively
    describe this phenomenon. Anomalous quantum effects have been predicted and
    some have been experimentally confirmed. A systematically truncated cluster-correlation
    expansion theory has been developed to account for the many-body correlations
    in nanoscale nuclear spin baths that are built up during electron spin decoherence.
    The theory has successfully predicted and explained a number of experimental
    results in a wide range of physical systems. In this review, we will cover
    this recent progress. The limitations of the present quantum many-body theories
    and possible directions for future development will also be discussed.},
  author={Yang, Wen and Ma, Wen-Long and Liu, Ren-Bao},
  date-added={2017-08-18 12:33:07 +0000},
  date-modified={2017-08-18 12:33:36 +0000},
  doi={10.1088/0034-4885/80/1/016001},
  journal={Rep. Prog. Phys.},
  journal-full={Reports on progress in physics. Physical Society (Great Britain)},
  number={1},
  pages={016001},
  pmid={27811398},
  pst={ppublish},
  title={Quantum many-body theory for electron spin decoherence in nanoscale nuclear
    spin baths},
  volume={80},
  year={2017},
  bdsk-url-1={http://dx.doi.org/10.1088/0034-4885/80/1/016001}
}

@article{Dobrovitski2003,
  abstract={We demonstrate that the Chebyshev expansion method is a very efficient
    numerical tool for studying spin-bath decoherence of quantum systems. We consider
    two typical problems arising in studying decoherence of quantum systems consisting
    of a few coupled spins: (i) determining the pointer states of the system and
    (ii) determining the temporal decay of quantum oscillations. As our results
    demonstrate, for determining the pointer states, the Chebyshev-based scheme
    is at least a factor of 8 faster than existing algorithms based on the Suzuki-Trotter
    decomposition. For problems of the second type, the Chebyshev-based approach
    is 3-4 times faster than the Suzuki-Trotter-based schemes. This conclusion
    holds qualitatively for a wide spectrum of systems, with different spin baths
    and different Hamiltonians.},
  author={Dobrovitski, V V and {De Raedt}, H A},
  date-added={2017-08-18 10:20:29 +0000},
  date-modified={2017-08-18 10:21:07 +0000},
  doi={10.1103/PhysRevE.67.056702},
  journal={Phys. Rev. E},
  journal-full={Physical review. E, Statistical, nonlinear, and soft matter physics},
  number={5 Pt 2},
  pages={056702},
  pmid={12786317},
  pst={ppublish},
  title={Efficient scheme for numerical simulations of the spin-bath decoherence},
  volume={67},
  year={2003},
  bdsk-url-1={http://dx.doi.org/10.1103/PhysRevE.67.056702}
}

@article{Sousa2003,
  author={R. {de Sousa} and S. {Das Sarma}},
  date-added={2017-08-18 10:01:29 +0000},
  date-modified={2017-08-18 10:02:25 +0000},
  doi={10.1103/PhysRevB.68.115322},
  journal={Phys. Rev. B},
  pages={115322},
  title={Theory of nuclear-induced spectral diffusion: Spin decoherence of phosphorus
    donors in Si and GaAs quantum dots},
  volume={68},
  year={2003},
  bdsk-url-1={http://dx.doi.org/10.1103/PhysRevB.68.115322}
}

@article{Hanson2007,
  author={R. Hanson and L. P. Kouwenhoven and J. R. Petta and S. Tarucha and L.
    M. K. Vandersypen},
  doi={10.1103/RevModPhys.79.1217},
  journal={Rev. Mod. Phys.},
  month={oct},
  number={4},
  owner={Mehdi Abdi},
  pages={1217},
  publisher={American Physical Society ({APS})},
  title={Spins in few-electron quantum dots},
  volume={79},
  year={2007},
  bdsk-url-1={http://dx.doi.org/10.1103/RevModPhys.79.1217}
}

@article{Witzel2005,
  author={W. M. Witzel and Rogerio de Sousa and S. Das Sarma},
  doi={10.1103/PhysRevB.72.161306},
  journal={Phys. Rev. B},
  month={oct},
  number={16},
  owner={Mehdi Abdi},
  pages={161306},
  publisher={American Physical Society ({APS})},
  title={Quantum theory of spectral-diffusion-induced electron spin decoherence},
  volume={72},
  year={2005},
  bdsk-url-1={http://dx.doi.org/10.1103/PhysRevB.72.161306}
}

@article{Lee1985,
  author={Patrick A. Lee and T. V. Ramakrishnan},
  doi={10.1103/RevModPhys.57.287},
  journal={Rev. Mod. Phys.},
  month={apr},
  number={2},
  owner={Mehdi Abdi},
  pages={287--337},
  publisher={American Physical Society ({APS})},
  title={Disordered electronic systems},
  volume={57},
  year={1985},
  bdsk-url-1={http://dx.doi.org/10.1103/RevModPhys.57.287}
}

@article{Degenfeld2014,
  author={Peter Degenfeld-Schonburg and Michael J. Hartmann},
  doi={10.1103/PhysRevB.89.245108},
  journal={Phys. Rev. B},
  month={jun},
  number={24},
  owner={Mehdi Abdi},
  pages={245108},
  publisher={American Physical Society ({APS})},
  title={Self-consistent projection operator theory for quantum many-body systems},
  volume={89},
  year={2014},
  bdsk-url-1={http://dx.doi.org/10.1103/PhysRevB.89.245108}
}

@article{Puebla2016,
  author={Ricardo Puebla and Jorge Casanova and Martin B Plenio},
  doi={10.1088/1367-2630/18/11/113039},
  journal={New J. Phys.},
  month={nov},
  number={11},
  owner={Mehdi Abdi},
  pages={113039},
  publisher={{IOP} Publishing},
  title={A robust scheme for the implementation of the quantum Rabi model in trapped
    ions},
  volume={18},
  year={2016},
  bdsk-url-1={http://dx.doi.org/10.1088/1367-2630/18/11/113039}
}

@article{Cai2012,
  author={J-M Cai and B Naydenov and R Pfeiffer and L P McGuinness and K D Jahnke
    and F Jelezko and M B Plenio and A Retzker},
  doi={10.1088/1367-2630/14/11/113023},
  journal={New J. Phys.},
  month={nov},
  number={11},
  owner={Mehdi Abdi},
  pages={113023},
  publisher={{IOP} Publishing},
  title={Robust dynamical decoupling with concatenated continuous driving},
  volume={14},
  year={2012},
  bdsk-url-1={http://dx.doi.org/10.1088/1367-2630/14/11/113023}
}

@article{Khaetskii2003,
  author={Alexander Khaetskii and Daniel Loss and Leonid Glazman},
  doi={10.1103/PhysRevB.67.195329},
  journal={Phys. Rev. B},
  month={may},
  number={19},
  owner={Mehdi Abdi},
  pages={195329},
  publisher={American Physical Society ({APS})},
  title={Electron spin evolution induced by interaction with nuclei in a quantum
    dot},
  volume={67},
  year={2003},
  bdsk-url-1={http://dx.doi.org/10.1103/PhysRevB.67.195329}
}

@book{Breuer2007,
  author={Heinz-Peter Breuer and Francesco Petruccione},
  date={2007-02-11},
  ean={9780199213900},
  isbn={978-0199213900},
  owner={Mehdi Abdi},
  publisher={Oxford University Press},
  title={The Theory of Open Quantum Systems},
  url={http://www.ebook.de/de/product/6212122/heinz_peter_breuer_francesco_petruccione_the_theory_of_open_quantum_systems.html},
  year={2007},
  bdsk-url-1={http://www.ebook.de/de/product/6212122/heinz_peter_breuer_francesco_petruccione_the_theory_of_open_quantum_systems.html}
}

@Article{Fernandez2018b,
  author={Fern{\'a}ndez-Acebal, P and Plenio, Martin B},
  journal={Sci. Rep.},
  title={Sensing phases of water via nitrogen-vacancy centres in diamond},
  year={2018},
  number={1},
  pages={13453},
  volume={8},
  bdsk-url-1={https://doi.org/10.1038/s41598-018-31745-3},
  date-modified={2022-05-15 08:40:18 +0430},
  doi={10.1038/s41598-018-31745-3}
}

@Article{Holstein1940,
  author={Holstein, T and Primakoff, Hl},
  journal={Phys. Rev.},
  title={Field dependence of the intrinsic domain magnetization of a ferromagnet},
  year={1940},
  number={12},
  pages={1098},
  volume={58},
  bdsk-url-1={https://doi.org/10.1103/PhysRev.58.1098},
  date-modified={2022-05-15 08:41:01 +0430},
  doi={10.1103/PhysRev.58.1098},
  publisher={APS}
}

@Article{Fanchini2014,
  author        = {Fanchini, Felipe F and Karpat, Goktug and {\c{C}}akmak, Baris and Castelano, LK and Aguilar, GH and Far{\'\i}as, O Jim{\'e}nez and Walborn, SP and Ribeiro, PH Souto and De Oliveira, MC},
  journal       = {Phys. Rev. Lett.},
  title         = {Non-Markovianity through accessible information},
  year          = {2014},
  number        = {21},
  pages         = {210402},
  volume        = {112},
  date-modified = {2022-05-15 08:39:29 +0430},
  publisher     = {APS},
}

@article{Loretz2017,
  author={Loretz, M. and Takahashi, H. and Segawa, T. F. and Boss, J. M. and Degen,
    C. L.},
  doi={10.1103/PhysRevB.95.064413},
  issue={6},
  journal={Phys. Rev. B},
  month={Feb},
  numpages={6},
  pages={064413},
  publisher={American Physical Society},
  title={Optical hyperpolarization of nitrogen donor spins in bulk diamond},
  url={https://link.aps.org/doi/10.1103/PhysRevB.95.064413},
  volume={95},
  year={2017},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevB.95.064413},
  bdsk-url-2={https://doi.org/10.1103/PhysRevB.95.064413}
}

@article{Bucher2020,
  author={Bucher, Dominik B. and Glenn, David R. and Park, Hongkun and Lukin, Mikhail
    D. and Walsworth, Ronald L.},
  doi={10.1103/PhysRevX.10.021053},
  issue={2},
  journal={Phys. Rev. X},
  month={Jun},
  numpages={9},
  pages={021053},
  publisher={American Physical Society},
  title={Hyperpolarization-Enhanced NMR Spectroscopy with Femtomole Sensitivity
    Using Quantum Defects in Diamond},
  url={https://link.aps.org/doi/10.1103/PhysRevX.10.021053},
  volume={10},
  year={2020},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevX.10.021053},
  bdsk-url-2={https://doi.org/10.1103/PhysRevX.10.021053}
}

@article{Tetienne2021a,
  author={Tetienne, J.-P. and Hall, L. T. and Healey, A. J. and White, G. A. L.
    and Sani, M.-A. and Separovic, F. and Hollenberg, L. C. L.},
  date-modified={2022-05-15 08:42:50 +0430},
  doi={10.1103/PhysRevB.103.014434},
  issue={1},
  journal={Phys. Rev. B},
  month={Jan},
  numpages={17},
  pages={014434},
  publisher={American Physical Society},
  title={Prospects for nuclear spin hyperpolarization of molecular samples using
    nitrogen-vacancy centers in diamond},
  url={https://link.aps.org/doi/10.1103/PhysRevB.103.014434},
  volume={103},
  year={2021},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevB.103.014434},
  bdsk-url-2={https://doi.org/10.1103/PhysRevB.103.014434}
}

@article{Green2017,
  author={Green, B. L. and Breeze, B. G. and Rees, G. J. and Hanna, J. V. and Chou,
    J.-P. and Iv\'ady, V. and Gali, A. and Newton, M. E.},
  doi={10.1103/PhysRevB.96.054101},
  issue={5},
  journal={Phys. Rev. B},
  month={Aug},
  numpages={8},
  pages={054101},
  publisher={American Physical Society},
  title={All-optical hyperpolarization of electron and nuclear spins in diamond},
  url={https://link.aps.org/doi/10.1103/PhysRevB.96.054101},
  volume={96},
  year={2017},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevB.96.054101},
  bdsk-url-2={https://doi.org/10.1103/PhysRevB.96.054101}
}

@article{Griffin2010,
  author={Griffin, R. G. and Prisner, T. F.},
  doi={10.1039/C0CP90019B},
  issue={22},
  journal={Phys. Chem. Chem. Phys.},
  pages={5737-5740},
  publisher={The Royal Society of Chemistry},
  title={High field dynamic nuclear polarization-the renaissance},
  url={http://dx.doi.org/10.1039/C0CP90019B},
  volume={12},
  year={2010},
  bdsk-url-1={http://dx.doi.org/10.1039/C0CP90019B}
}

@Article{Thankamony2017,
  author={Aany Sofia {Lilly Thankamony} and Johannes J. Wittmann and Monu Kaushik
    and Bjorn Corzilius},
  journal={Prog. Nuc. Mag. Res. Sp.},
  title={Dynamic nuclear polarization for sensitivity enhancement in modern solid-state
    NMR},
  year={2017},
  issn={0079-6565},
  pages={120-195},
  volume={102-103},
  abstract={The field of dynamic nuclear polarization has undergone tremendous
    developments and diversification since its inception more than 6 decades ago.
    In this review we provide an in-depth overview of the relevant topics involved
    in DNP-enhanced MAS NMR spectroscopy. This includes the theoretical description
    of DNP mechanisms as well as of the polarization transfer pathways that can
    lead to a uniform or selective spreading of polarization between nuclear spins.
    Furthermore, we cover historical and state-of-the art aspects of dedicated
    instrumentation, polarizing agents, and optimization techniques for efficient
    MAS DNP. Finally, we present an extensive overview on applications in the fields
    of structural biology and materials science, which underlines that MAS DNP
    has moved far beyond the proof-of-concept stage and has become an important
    tool for research in these fields.},
  bdsk-url-1={https://www.sciencedirect.com/science/article/pii/S0079656517300201},
  bdsk-url-2={https://doi.org/10.1016/j.pnmrs.2017.06.002},
  doi={https://doi.org/10.1016/j.pnmrs.2017.06.002},
  url={https://www.sciencedirect.com/science/article/pii/S0079656517300201}
}

@Article{Gallagher2008,
  author={Gallagher, Ferdia A and Kettunen, Mikko I and Day, Sam E and Hu, De-En
    and Ardenkjaer-Larsen, Jan Henrik and Zandt, Ren{\'e} and Jensen, Pernille
    R and Karlsson, Magnus and Golman, Klaes and Lerche, Mathilde H and others},
  journal={Nature},
  title={Magnetic resonance imaging of pH in vivo using hyperpolarized ${}^{13}$C-labelled
    bicarbonate},
  year={2008},
  number={7197},
  pages={940--943},
  volume={453},
  bdsk-url-1={{\%}22https://doi.org/10.1038/nature07017{\%}22},
  doi={"https://doi.org/10.1038/nature07017"},
  publisher={Nature Publishing Group},
  url={"https://doi.org/10.1038/nature07017"}
}

@Article{Bowen2008,
  author={Bowen, Sean and Hilty, Christian},
  journal={Angew. Chem. Int. Ed.},
  title={Time-Resolved Dynamic Nuclear Polarization Enhanced NMR Spectroscopy},
  year={2008},
  number={28},
  pages={5235-5237},
  volume={47},
  abstract={The sensitive touch: Sensitivity constraints in NMR spectroscopy typically
    call for long measurement times. Hyperpolarization can enhance the time resolution
    of NMR spectroscopy by removing the need for signal averaging. Reactions such
    as enzyme catalysis can be followed in real time by hyperpolarized NMR spectroscopy
    through reduction in the intensity of the substrate resonance as well as the
    appearance of product resonances (see picture).},
  bdsk-url-1={https://onlinelibrary.wiley.com/doi/abs/10.1002/anie.200801492},
  bdsk-url-2={https://doi.org/10.1002/anie.200801492},
  doi={https://doi.org/10.1002/anie.200801492},
  keywords={enzyme catalysis, hyperpolarization, kinetics, NMR spectroscopy},
  url={https://onlinelibrary.wiley.com/doi/abs/10.1002/anie.200801492}
}

@Article{Cunningham2016,
  author={Charles H. Cunningham and Justin Y.C. Lau and Albert P. Chen and Benjamin
    J. Geraghty and William J. Perks and Idan Roifman and Graham A. Wright and
    Kim A. Connelly},
  journal={Circ. Res.},
  title={Hyperpolarized ${}^{13}$C Metabolic MRI of the Human Heart},
  year={2016},
  number={11},
  pages={1177-1182},
  volume={119},
  bdsk-url-1={https://www.ahajournals.org/doi/abs/10.1161/CIRCRESAHA.116.309769},
  url={https://www.ahajournals.org/doi/abs/10.1161/CIRCRESAHA.116.309769}
}

@Article{Foletti2009,
  author={Foletti, Sandra and Bluhm, Hendrik and Mahalu, Diana and Umansky, Vladimir
    and Yacoby, Amir},
  journal={Nat. Phys.},
  title={Universal quantum control of two-electron spin quantum bits using dynamic
    nuclear polarization},
  year={2009},
  number={12},
  pages={903--908},
  volume={5},
  bdsk-url-1={{\%}22https://doi.org/10.1038/nphys1424{\%}22},
  doi={"https://doi.org/10.1038/nphys1424"},
  publisher={Nature Publishing Group},
  url={"https://doi.org/10.1038/nphys1424"}
}

@Article{Natterer1997,
  author={Johannes Natterer and Joachim Bargon},
  journal={Prog. Nuc. Mag. Res. Sp.},
  title={Parahydrogen induced polarization},
  year={1997},
  issn={0079-6565},
  number={4},
  pages={293-315},
  volume={31},
  bdsk-url-1={https://www.sciencedirect.com/science/article/pii/S0079656597000071},
  bdsk-url-2={https://doi.org/10.1016/S0079-6565(97)00007-1},
  doi={https://doi.org/10.1016/S0079-6565(97)00007-1},
  keywords={PASADENA, PHIP, ALTADENA, Para- and orthohydrogen, Homogeneous hydrogenation,
    Hydrides, Coherence transfer, Hydrogenation mechanisms, Signal enhancement,
    NMR pulse sequences},
  url={https://www.sciencedirect.com/science/article/pii/S0079656597000071}
}

@Article{Hovener2018,
  author={H{\"o}vener, Jan-Bernd and Pravdivtsev, Andrey N. and Kidd, Bryce and
    Bowers, C. Russell and Gl{\"o}ggler, Stefan and Kovtunov, Kirill V. and Plaumann,
    Markus and Katz-Brull, Rachel and Buckenmaier, Kai and Jerschow, Alexej and
    Reineri, Francesca and Theis, Thomas and Shchepin, Roman V. and Wagner, Shawn
    and Bhattacharya, Pratip and Zacharias, Niki M. and Chekmenev, Eduard Y.},
  journal={Angew. Chem. Int. Ed.},
  title={Parahydrogen-Based Hyperpolarization for Biomedicine},
  year={2018},
  number={35},
  pages={11140-11162},
  volume={57},
  bdsk-url-1={https://onlinelibrary.wiley.com/doi/abs/10.1002/anie.201711842},
  bdsk-url-2={https://doi.org/10.1002/anie.201711842},
  doi={https://doi.org/10.1002/anie.201711842},
  keywords={hyperpolarization, magnetic resonance imaging, NMR spectroscopy, parahydrogen},
  url={https://onlinelibrary.wiley.com/doi/abs/10.1002/anie.201711842}
}

@article{Walker1998,
  author={Walker, Thad G. and Happer, William},
  doi={10.1103/RevModPhys.69.629},
  issue={2},
  journal={Rev. Mod. Phys.},
  month={Apr},
  numpages={0},
  pages={629--642},
  publisher={American Physical Society},
  title={Spin-exchange optical pumping of noble-gas nuclei},
  url={https://link.aps.org/doi/10.1103/RevModPhys.69.629},
  volume={69},
  year={1997},
  bdsk-url-1={https://link.aps.org/doi/10.1103/RevModPhys.69.629},
  bdsk-url-2={https://doi.org/10.1103/RevModPhys.69.629}
}

@Article{Navon1996,
  author={G. Navon and Y.-Q. and T. R{\~o}{\~o}m and S. Appelt and R. E. Taylor
    and A. Pines},
  journal={Science},
  title={Enhancement of Solution NMR and MRI with Laser-Polarized Xenon},
  year={1996},
  number={5257},
  pages={1848-1851},
  volume={271},
  abstract={Optical pumping with laser light can be used to polarize the nuclear
    spins of gaseous xenon-129. When hyperpolarized xenon-129 is dissolved in liquids,
    a time-dependent departure of the proton spin polarization from its thermal
    equilibrium is observed. The variation of the magnetization is an unexpected
    manifestation of the nuclear Overhauser effect, a consequence of cross-relaxation
    between the spins of solution protons and dissolved xenon-129. Time-resolved
    magnetic resonance images of both nuclei in solution show that the proton magnetization
    is selectively perturbed in regions containing spin-polarized xenon-129. This
    effect could find use in nuclear magnetic resonance spectroscopy of surfaces
    and proteins and in magnetic resonance imaging.},
  bdsk-url-1={https://www.science.org/doi/abs/10.1126/science.271.5257.1848},
  bdsk-url-2={https://doi.org/10.1126/science.271.5257.1848},
  doi={10.1126/science.271.5257.1848},
  url={https://www.science.org/doi/abs/10.1126/science.271.5257.1848}
}

@article{Villazon2021,
  author={Villazon, Tamiro and Claeys, Pieter W. and Polkovnikov, Anatoli and Chandran,
    Anushya},
  doi={10.1103/PhysRevB.103.075118},
  issue={7},
  journal={Phys. Rev. B},
  month={Feb},
  numpages={21},
  pages={075118},
  publisher={American Physical Society},
  title={Shortcuts to dynamic polarization},
  url={https://link.aps.org/doi/10.1103/PhysRevB.103.075118},
  volume={103},
  year={2021},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevB.103.075118},
  bdsk-url-2={https://doi.org/10.1103/PhysRevB.103.075118}
}

@Article{Abragam1978,
  author={A Abragam and M Goldman},
  journal={Rep. Progr. Phys.},
  title={Principles of dynamic nuclear polarisation},
  year={1978},
  month={mar},
  number={3},
  pages={395--467},
  volume={41},
  abstract={After a general introduction, two sections are devoted to a survey
    of the theories of spin temperature and of nuclear relaxation in solids. This
    is followed by a short section on the so-called well-resolved solid effect,
    and a much more detailed one on DNP by thermal mixing in the non-linear low
    spin-temperature domain. One then analyses the various methods of measurement
    of the nuclear polarisation, as well as an indirect method of detecting the
    electronic resonance based on the existence of large nuclear polarisations.
    The final section describes briefly several applications of dynamic nuclear
    polarisation.},
  bdsk-url-1={https://doi.org/10.1088/0034-4885/41/3/002},
  doi={10.1088/0034-4885/41/3/002},
  publisher={{IOP} Publishing},
  url={https://doi.org/10.1088/0034-4885/41/3/002}
}

@article{Gullans2013,
  author={Gullans, M. and Krich, J. J. and Taylor, J. M. and Halperin, B. I. and
    Lukin, M. D.},
  doi={10.1103/PhysRevB.88.035309},
  issue={3},
  journal={Phys. Rev. B},
  month={Jul},
  numpages={14},
  pages={035309},
  publisher={American Physical Society},
  title={Preparation of nonequilibrium nuclear spin states in double quantum dots},
  url={https://link.aps.org/doi/10.1103/PhysRevB.88.035309},
  volume={88},
  year={2013},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevB.88.035309},
  bdsk-url-2={https://doi.org/10.1103/PhysRevB.88.035309}
}

@article{Lai2006,
  author={Lai, C. W. and Maletinsky, P. and Badolato, A. and Imamoglu, A.},
  doi={10.1103/PhysRevLett.96.167403},
  issue={16},
  journal={Phys. Rev. Lett.},
  month={Apr},
  numpages={4},
  pages={167403},
  publisher={American Physical Society},
  title={Knight-Field-Enabled Nuclear Spin Polarization in Single Quantum Dots},
  url={https://link.aps.org/doi/10.1103/PhysRevLett.96.167403},
  volume={96},
  year={2006},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevLett.96.167403},
  bdsk-url-2={https://doi.org/10.1103/PhysRevLett.96.167403}
}

@article{Urbaszek2013,
  author={Urbaszek, Bernhard and Marie, Xavier and Amand, Thierry and Krebs, Olivier
    and Voisin, Paul and Maletinsky, Patrick and H\"ogele, Alexander and Imamoglu,
    Atac},
  doi={10.1103/RevModPhys.85.79},
  issue={1},
  journal={Rev. Mod. Phys.},
  month={Jan},
  numpages={0},
  pages={79--133},
  publisher={American Physical Society},
  title={Nuclear spin physics in quantum dots: An optical investigation},
  url={https://link.aps.org/doi/10.1103/RevModPhys.85.79},
  volume={85},
  year={2013},
  bdsk-url-1={https://link.aps.org/doi/10.1103/RevModPhys.85.79},
  bdsk-url-2={https://doi.org/10.1103/RevModPhys.85.79}
}

@Article{Lee2016,
  author={Daniel Lee and Eric Bouleau and Pierre Saint-Bonnet and Sabine Hediger
    and Ga{\"e}l {De Pa{\"e}pe}},
  journal={J. Magn. Reson.},
  title={Ultra-low temperature MAS-DNP},
  year={2016},
  issn={1090-7807},
  note={Hyperpolarized NMR Comes of Age},
  pages={116-124},
  volume={264},
  bdsk-url-1={https://www.sciencedirect.com/science/article/pii/S1090780715003092},
  bdsk-url-2={https://doi.org/10.1016/j.jmr.2015.12.010},
  doi={https://doi.org/10.1016/j.jmr.2015.12.010},
  keywords={Dynamic nuclear polarization, Magic angle spinning, Solid-state NMR,
    Cryogenic helium, Helium sample spinning},
  url={https://www.sciencedirect.com/science/article/pii/S1090780715003092}
}

@Article{Kaplan2015,
  author={Kaplan, Mohammed and Cukkemane, Abhishek and Van Zundert, Gydo CP and
    Narasimhan, Siddarth and Dani{\"e}ls, Mark and Mance, Deni and Waksman, Gabriel
    and Bonvin, Alexandre MJJ and Fronzes, R{\'e}mi and Folkers, Gert E and others},
  journal={Nat. Methods},
  title={Probing a cell-embedded megadalton protein complex by DNP-supported solid-state
    NMR},
  year={2015},
  number={7},
  pages={649--652},
  volume={12},
  bdsk-url-1={https://doi.org/10.1038/nmeth.3406},
  doi={https://doi.org/10.1038/nmeth.3406},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/nmeth.3406}
}

@article{King2010,
  author={King, Jonathan P. and Coles, Patrick J. and Reimer, Jeffrey A.},
  doi={10.1103/PhysRevB.81.073201},
  issue={7},
  journal={Phys. Rev. B},
  month={Feb},
  numpages={4},
  pages={073201},
  publisher={American Physical Society},
  title={Optical polarization of $^{13}\text{C}$ nuclei in diamond through nitrogen
    vacancy centers},
  url={https://link.aps.org/doi/10.1103/PhysRevB.81.073201},
  volume={81},
  year={2010},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevB.81.073201},
  bdsk-url-2={https://doi.org/10.1103/PhysRevB.81.073201}
}

@article{Pagliero2018,
  author={Pagliero, Daniela and Rao, K. R. Koteswara and Zangara, Pablo R. and
    Dhomkar, Siddharth and Wong, Henry H. and Abril, Andrea and Aslam, Nabeel and
    Parker, Anna and King, Jonathan and Avalos, Claudia E. and Ajoy, Ashok and
    Wrachtrup, Joerg and Pines, Alexander and Meriles, Carlos A.},
  doi={10.1103/PhysRevB.97.024422},
  issue={2},
  journal={Phys. Rev. B},
  month={Jan},
  numpages={12},
  pages={024422},
  publisher={American Physical Society},
  title={Multispin-assisted optical pumping of bulk $^{13}\mathrm{C}$ nuclear spin
    polarization in diamond},
  url={https://link.aps.org/doi/10.1103/PhysRevB.97.024422},
  volume={97},
  year={2018},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevB.97.024422},
  bdsk-url-2={https://doi.org/10.1103/PhysRevB.97.024422}
}

@Article{Ajoy2018,
  author={Ashok Ajoy and Kristina Liu and Raffi Nazaryan and Xudong Lv and Pablo
    R. Zangara and Benjamin Safvati and Guoqing Wang and Daniel Arnold and Grace
    Li and Arthur Lin and Priyanka Raghavan and Emanuel Druga and Siddharth Dhomkar
    and Daniela Pagliero and Jeffrey A. Reimer and Dieter Suter and Carlos A. Meriles
    and Alexander Pines},
  journal={Sci. Adv.},
  title={Orientation-independent room temperature optical $^{13}\mathrm{C}$ hyperpolarization
    in powdered diamond},
  year={2018},
  number={5},
  pages={5492},
  volume={4},
  abstract={@Commentjabref-meta: databaseType:bibtex;},
  bdsk-url-1={https://www.science.org/doi/abs/10.1126/sciadv.aar5492},
  bdsk-url-2={https://doi.org/10.1126/sciadv.aar5492},
  doi={10.1126/sciadv.aar5492},
  url={https://www.science.org/doi/abs/10.1126/sciadv.aar5492}
}

@article{Abdi2018,
  author={Abdi, Mehdi and Chou, Jyh-Pin and Gali, Adam and Plenio, Martin B.},
  doi={10.1021/acsphotonics.7b01442},
  journal={ACS Photonics},
  number={5},
  pages={1967-1976},
  title={Color Centers in Hexagonal Boron Nitride Monolayers: A Group Theory and
    Ab Initio Analysis},
  url={https://doi.org/10.1021/acsphotonics.7b01442},
  volume={5},
  year={2018},
  bdsk-url-1={https://doi.org/10.1021/acsphotonics.7b01442}
}

@article{Abdi2017,
  author={Mehdi Abdi and Myung-Joong Hwang and Mortaza Aghtar and Martin B. Plenio},
  doi={10.1103/physrevlett.119.233602},
  journal={Phys. Rev. Lett.},
  month={dec},
  number={23},
  owner={Mehdi Abdi},
  pages={233602},
  publisher={American Physical Society ({APS})},
  title={Spin-Mechanical Scheme with Color Centers in Hexagonal Boron Nitride Membranes},
  volume={119},
  year={2017},
  bdsk-url-1={https://doi.org/10.1103/physrevlett.119.233602}
}

@article{Abdi2019,
  author={Mehdi Abdi and Martin B. Plenio},
  date-added={2021-01-16 09:39:24 +0330},
  date-modified={2021-01-16 09:39:24 +0330},
  doi={10.1103/physrevlett.122.023602},
  journal={Phys. Rev. Lett.},
  month={jan},
  number={2},
  pages={023602},
  publisher={American Physical Society ({APS})},
  title={Quantum Effects in a Mechanically Modulated Single-Photon Emitter},
  volume={122},
  year={2019},
  bdsk-url-1={https://doi.org/10.1103/physrevlett.122.023602}
}

@Article{Henshaw2019,
  author={Henshaw, Jacob and Pagliero, Daniela and Zangara, Pablo R. and Franzoni,
    Mar{\'\i}a B. and Ajoy, Ashok and Acosta, Rodolfo H. and Reimer, Jeffrey A.
    and Pines, Alexander and Meriles, Carlos A.},
  journal={Proc. Natl. Acad. Sci.},
  title={Carbon-13 dynamic nuclear polarization in diamond via a microwave-free
    integrated cross effect},
  year={2019},
  issn={0027-8424},
  number={37},
  pages={18334--18340},
  volume={116},
  abstract={Optical spin pumping of color centers promises to revolutionize the
    practice of nuclear magnetic resonance via efficient dynamic nuclear polarization
    protocols. Significant progress has been attained with systems such as the
    nitrogen-vacancy (NV) center in diamond, but extreme spectral broadening and
    nuclear spin-lattice relaxation from coexisting paramagnetic defects are hurdles
    still difficult to circumvent. The present technique addresses both issues
    through the implementation of magnetic-field-sweep{\textendash}induced NV cross-relaxation
    with ancilla point defects, here acting as proxies to mediate the transfer
    of polarization to the nuclear spin ensemble. The governing spin dynamics is
    robust to field misalignment and ideally suited for shallow NVs, indirectly
    coupled to outside nuclei through paramagnetic defects at the diamond surface.Color-center{\textendash}hosting
    semiconductors are emerging as promising source materials for low-field dynamic
    nuclear polarization (DNP) at or near room temperature, but hyperfine broadening,
    susceptibility to magnetic field heterogeneity, and nuclear spin relaxation
    induced by other paramagnetic defects set practical constraints difficult to
    circumvent. Here, we explore an alternate route to color-center{\textendash}assisted
    DNP using nitrogen-vacancy (NV) centers in diamond coupled to substitutional
    nitrogen impurities, the so-called P1 centers. Working near the level anticrossing
    condition{\textemdash}where the P1 Zeeman splitting matches one of the NV spin
    transitions{\textemdash}we demonstrate efficient microwave-free 13C DNP through
    the use of consecutive magnetic field sweeps and continuous optical excitation.
    The amplitude and sign of the polarization can be controlled by adjusting the
    low-to-high and high-to-low magnetic field sweep rates in each cycle so that
    one is much faster than the other. By comparing the 13C DNP response for different
    crystal orientations, we show that the process is robust to magnetic field/NV
    misalignment, a feature that makes the present technique suitable to diamond
    powders and settings where the field is heterogeneous. Applications to shallow
    NVs could capitalize on the greater physical proximity between surface paramagnetic
    defects and outer nuclei to efficiently polarize target samples in contact
    with the diamond crystal.},
  bdsk-url-1={https://www.pnas.org/content/116/37/18334},
  bdsk-url-2={https://doi.org/10.1073/pnas.1908780116},
  doi={10.1073/pnas.1908780116},
  publisher={National Academy of Sciences},
  url={https://www.pnas.org/content/116/37/18334}
}

@Article{Broadway2018,
  author={Broadway, David A and Tetienne, Jean-Philippe and Stacey, Alastair and
    Wood, James DA and Simpson, David A and Hall, Liam T and Hollenberg, Lloyd
    CL},
  journal={Nat. Commun.},
  title={Quantum probe hyperpolarisation of molecular nuclear spins},
  year={2018},
  pages={1246},
  volume={9},
  bdsk-url-1={https://doi.org/10.1038/s41467-018-03578-1},
  doi={https://doi.org/10.1038/s41467-018-03578-1},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/s41467-018-03578-1}
}

@Article{Tran2016,
  author={Tran, Toan Trong and Bray, Kerem and Ford, Michael J and Toth, Milos
    and Aharonovich, Igor},
  journal={Nat. Nanotechnol.},
  title={Quantum emission from hexagonal boron nitride monolayers},
  year={2016},
  number={1},
  pages={37--41},
  volume={11},
  bdsk-url-1={https://doi.org/10.1038/nnano.2015.242},
  doi={https://doi.org/10.1038/nnano.2015.242},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/nnano.2015.242}
}

@Article{Sajid2020,
  author={A Sajid and Michael J Ford and Jeffrey R Reimers},
  journal={Rep. Progr. Phys.},
  title={Single-photon emitters in hexagonal boron nitride: a review of progress},
  year={2020},
  month={mar},
  number={4},
  pages={044501},
  volume={83},
  bdsk-url-1={https://doi.org/10.1088/1361-6633/ab6310},
  doi={10.1088/1361-6633/ab6310},
  publisher={{IOP} Publishing},
  url={https://doi.org/10.1088/1361-6633/ab6310}
}

@article{Gyamfi2019,
  author={Gyamfi, JA},
  journal={arXiv preprint arXiv:1907.07122},
  title={An Introduction to the Holstein-Primakoff Transformation, with Applications
    in Magnetic Resonance},
  url={https://arxiv.org/abs/1907.07122},
  year={2019},
  bdsk-url-1={https://arxiv.org/abs/1907.07122}
}

@article{Abad2016,
  author={Abad, Tahereh and Karimipour, Vahid},
  doi={10.1103/PhysRevB.93.195127},
  issue={19},
  journal={Phys. Rev. B},
  month={May},
  numpages={5},
  pages={195127},
  publisher={American Physical Society},
  title={Scaling of macroscopic superpositions close to a quantum phase transition},
  url={https://link.aps.org/doi/10.1103/PhysRevB.93.195127},
  volume={93},
  year={2016},
  bdsk-url-1={https://link.aps.org/doi/10.1103/PhysRevB.93.195127},
  bdsk-url-2={https://doi.org/10.1103/PhysRevB.93.195127}
}

@Article{Lieb1961,
  author={Elliott Lieb and Theodore Schultz and Daniel Mattis},
  journal={Ann. Phys.},
  title={Two soluble models of an antiferromagnetic chain},
  year={1961},
  issn={0003-4916},
  number={3},
  pages={407-466},
  volume={16},
  abstract={Two genuinely quantum mechanical models for an antiferromagnetic linear
    chain with nearest neighbor interactions are constructed and solved exactly,
    in the sense that the ground state, all the elementary excitations and the
    free energy are found. A general formalism for calculating the instantaneous
    correlation between any two spins is developed and applied to the investigation
    of short- and long-range order. Both models show nonvanishing long-range order
    in the ground state for a range of values of a certain parameter {\^I}{\guillemotright}
    which is analogous to an anisotropy parameter in the Heisenberg model. A detailed
    comparison with the Heisenberg model suggests that the latter has no long-range
    order in the isotropic case but finite long-range order for any finite amount
    of anisotropy. The unreliability of variational methods for determining long-range
    order is emphasized. It is also shown that for spin 12 systems having rather
    general isotropic Heisenberg interactions favoring an antiferromagnetic ordering,
    the ground state is nondegenerate and there is no energy gap above the ground
    state in the energy spectrum of the total system.},
  bdsk-url-1={https://www.sciencedirect.com/science/article/pii/0003491661901154},
  bdsk-url-2={https://doi.org/10.1016/0003-4916(61)90115-4},
  date-modified={2022-05-15 08:41:30 +0430},
  doi={https://doi.org/10.1016/0003-4916(61)90115-4},
  url={https://www.sciencedirect.com/science/article/pii/0003491661901154}
}

@Article{Pfeuty1970,
  author={Pierre Pfeuty},
  journal={Ann. Phys.},
  title={The one-dimensional Ising model with a transverse field},
  year={1970},
  issn={0003-4916},
  number={1},
  pages={79-90},
  volume={57},
  abstract={The one-dimensional Ising model with a transverse field is solved exactly
    by transforming the set of Pauli operators to a new set of Fermi operators.
    The elementary excitations, the ground-state energy and the free energy are
    found. The instantaneous correlation function between any two spins is calculated
    and this model shows a finite long-range order in the ground state when the
    transverse field is less than a critical value.},
  bdsk-url-1={https://www.sciencedirect.com/science/article/pii/0003491670902708},
  bdsk-url-2={https://doi.org/10.1016/0003-4916(70)90270-8},
  date-modified={2022-05-15 08:41:52 +0430},
  doi={https://doi.org/10.1016/0003-4916(70)90270-8},
  url={https://www.sciencedirect.com/science/article/pii/0003491670902708}
}

@Article{Cassabois2016,
  author={Cassabois, Guillaume and Valvin, Pierre and Gil, Bernard},
  journal={Nat. Photonics},
  title={Hexagonal boron nitride is an indirect bandgap semiconductor},
  year={2016},
  number={4},
  pages={262--266},
  volume={10},
  bdsk-url-1={https://doi.org/10.1038/nphoton.2015.277},
  date-modified={2022-05-15 08:39:20 +0430},
  doi={https://doi.org/10.1038/nphoton.2015.277},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/nphoton.2015.277}
}

@article{healey2021q,
  author={Healey, AJ and Scholten, SC and Yang, T and Scott, JA and Abrahams, GJ
    and Robertson, IO and Hou, XF and Guo, YF and Rahman, S and Lu, Y and others},
  journal={arXiv preprint arXiv:2112.03488},
  title={Quantum microscopy with van der Waals heterostructures},
  url={https://arxiv.org/abs/2112.03488},
  year={2021}
}

@Article{Tetienne2021b,
  author={Tetienne, J.-P.},
  journal={Nat. Phys.},
  title={Quantum sensors go flat},
  year={2021},
  number={10},
  pages={1074--1075},
  volume={17},
  bdsk-url-1={https://doi.org/10.1038/s41567-021-01338-5},
  date-modified={2022-05-15 08:42:57 +0430},
  doi={https://doi.org/10.1038/s41567-021-01338-5},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/s41567-021-01338-5}
}

@article{Geim2013,
  author={Geim, Andre K and Grigorieva, Irina V},
  date-modified={2022-05-15 08:40:36 +0430},
  doi={https://doi.org/10.1038/nature12385},
  journal={Nature},
  number={7459},
  pages={419--425},
  publisher={Nature Publishing Group},
  title={Van der Waals heterostructures},
  url={https://doi.org/10.1038/nature12385},
  volume={499},
  year={2013},
  bdsk-url-1={https://doi.org/10.1038/nature12385}
}

@Article{Novoselov2016,
  author={K. S. Novoselov and A. Mishchenko and A. Carvalho and A. H. Castro Neto},
  journal={Science},
  title={2D materials and van der Waals heterostructures},
  year={2016},
  number={6298},
  pages={9439},
  volume={353},
  bdsk-url-1={https://www.science.org/doi/abs/10.1126/science.aac9439},
  bdsk-url-2={https://doi.org/10.1126/science.aac9439},
  date-modified={2022-05-15 09:05:08 +0430},
  doi={10.1126/science.aac9439},
  url={https://www.science.org/doi/abs/10.1126/science.aac9439}
}

@article{Gong2017,
  author={Gong, Cheng and Li, Lin and Li, Zhenglu and Ji, Huiwen and Stern, Alex
    and Xia, Yang and Cao, Ting and Bao, Wei and Wang, Chenzhe and Wang, Yuan and
    others},
  date-modified={2022-05-15 08:40:41 +0430},
  doi={https://doi.org/10.1038/nature22060},
  journal={Nature},
  number={7657},
  pages={265--269},
  publisher={Nature Publishing Group},
  title={Discovery of intrinsic ferromagnetism in two-dimensional van der Waals
    crystals},
  url={https://doi.org/10.1038/nature22060},
  volume={546},
  year={2017},
  bdsk-url-1={https://doi.org/10.1038/nature22060}
}

@article{huang2017,
  author={Huang, Bevin and Clark, Genevieve and Navarro-Moratalla, Efr{\'e}n and
    Klein, Dahlia R and Cheng, Ran and Seyler, Kyle L and Zhong, Ding and Schmidgall,
    Emma and McGuire, Michael A and Cobden, David H and others},
  doi={https://doi.org/10.1038/nature22391},
  journal={Nature},
  number={7657},
  pages={270--273},
  publisher={Nature Publishing Group},
  title={Layer-dependent ferromagnetism in a van der Waals crystal down to the
    monolayer limit},
  url={https://doi.org/10.1038/nature22391},
  volume={546},
  year={2017},
  bdsk-url-1={https://doi.org/10.1038/nature22391}
}

@Article{Li2019,
  author={Li, Hui and Ruan, Shuangchen and Zeng, Yu-Jia},
  journal={Adv. Mater.},
  title={Intrinsic Van Der Waals Magnetic Materials from Bulk to the 2D Limit:
    New Frontiers of Spintronics},
  year={2019},
  number={27},
  pages={1900065},
  volume={31},
  abstract={Abstract 2D van der Waals (vdW) magnets, which present intrinsic ferromagnetic/antiferromagnetic
    ground states at finite temperatures down to atomic-layer thicknesses, open
    a new horizon in materials science and enable the potential development of
    new spin-related applications. The layered structure of vdW magnets facilitates
    their atomic-layer cleavability and magnetic anisotropy, which counteracts
    spin fluctuations, thereby providing an ideal platform for theoretically and
    experimentally exploring magnetic phase transitions in the 2D limit. With reduced
    dimensions, the susceptibility of 2D magnets to a large variety of external
    stimuli also makes them more promising than their bulk counterpart in various
    device applications. Here, the current status of characterization and tuning
    of the magnetic properties of 2D vdW magnets, particularly the atomic-layer
    thickness, is presented. Various state-of-the-art optical and electrical techniques
    have been applied to reveal the magnetic states of 2D vdW magnets. Other emerging
    2D vdW magnets and future perspectives on the stacking strategy are also given;
    it is believed that they will excite more intensive research and provide unprecedented
    opportunities in the field of spintronics.},
  bdsk-url-1={https://onlinelibrary.wiley.com/doi/abs/10.1002/adma.201900065},
  bdsk-url-2={https://doi.org/10.1002/adma.201900065},
  date-modified={2022-05-15 08:41:22 +0430},
  doi={https://doi.org/10.1002/adma.201900065},
  keywords={2D vdW magnets, exfoliation, ferromagnetism, spintronics},
  url={https://onlinelibrary.wiley.com/doi/abs/10.1002/adma.201900065}
}

@Article{Liu2020,
  author={Liu, Shanshan and Yang, Ke and Liu, Wenqing and Zhang, Enze and Li, Zihan
    and Zhang, Xiaoqian and Liao, Zhiming and Zhang, Wen and Sun, Jiabao and Yang,
    Yunkun and others},
  journal={Natl. Sci. Rev.},
  title={Two-dimensional ferromagnetic superlattices},
  year={2020},
  number={4},
  pages={745--754},
  volume={7},
  bdsk-url-1={https://doi.org/10.1093/nsr/nwz205},
  date-modified={2022-05-15 08:41:39 +0430},
  doi={https://doi.org/10.1093/nsr/nwz205},
  publisher={Oxford University Press},
  url={https://doi.org/10.1093/nsr/nwz205}
}

@article{koehl2011,
  title={Room temperature coherent control of defect spin qubits in silicon carbide},
  author={Koehl, William F and Buckley, Bob B and Heremans, F Joseph and Calusine,
    Greg and Awschalom, David D},
  journal={Nature},
  volume={479},
  number={7371},
  pages={84--87},
  year={2011},
  publisher={Nature Publishing Group},
  doi={https://doi.org/10.1038/nature10562}
}

@article{widmann2015,
  title={Coherent control of single spins in silicon carbide at room temperature},
  author={Widmann, Matthias and Lee, Sang-Yun and Rendler, Torsten and Son, Nguyen
    Tien and Fedder, Helmut and Paik, Seoyoung and Yang, Li-Ping and Zhao, Nan
    and Yang, Sen and Booker, Ian and others},
  journal={Nat. Mater.},
  volume={14},
  number={2},
  pages={164--168},
  year={2015},
  publisher={Nature Publishing Group},
  doi={https://doi.org/10.1038/nmat4145}
}

@article{Falk2015,
  title={Optical Polarization of Nuclear Spins in Silicon Carbide},
  author={Falk, Abram L. and Klimov, Paul V. and Iv\'ady, Viktor and Sz\'asz, Kriszti\'an
    and Christle, David J. and Koehl, William F. and Gali, \'Ad\'am and Awschalom,
    David D.},
  journal={Phys. Rev. Lett.},
  volume={114},
  issue={24},
  pages={247603},
  numpages={6},
  year={2015},
  month={Jun},
  publisher={American Physical Society},
  doi={10.1103/PhysRevLett.114.247603},
  url={https://link.aps.org/doi/10.1103/PhysRevLett.114.247603}
}

@book{Baxter,
  title={Exactly solved models in statistical mechanics},
  author={R.J. Baxter},
  year={1982},
  publisher={London, Academic Press}
}

@book{nolting,
  title={Quantum theory of magnetism},
  author={Nolting, Wolfgang and Ramakanth, Anupuru},
  year={2009},
  publisher={Springer Science {\&} Business Media}
}

@Comment{jabref-meta: databaseType:bibtex;}

